Differentially Private Zeroth-Order Methods for Scalable Large Language Model Finetuning

Fine-tuning on task-specific datasets is a widely-embraced paradigm of harnessing the powerful capability of pretrained LLMs for various downstream tasks. Due to the popularity of LLMs fine-tuning and its accompanying privacy concerns, differentially private (DP) fine-tuning of pretrained LLMs has been widely used to safeguarding the privacy of task-specific datasets. Lying at the design core of DP LLM fine-tuning methods is the satisfactory tradeoff among privacy, utility, and scalability. Most existing methods build upon the seminal work of DP-SGD. Despite pushing the scalability of DP-SGD to its limit, DP-SGD-based fine-tuning methods are unfortunately limited by the inherent inefficiency of SGD. In this paper, we investigate the potential of DP zeroth-order methods for LLM pretraining, which avoids the scalability bottleneck of SGD by approximating the gradient with the more efficient zeroth-order gradient. Rather than treating the zeroth-order method as a drop-in replacement for SGD, this paper presents a comprehensive study both theoretically and empirically. First, we propose the stagewise DP zeroth-order method (DP-ZOSO) that dynamically schedules key hyperparameters. This design is grounded on the synergy between DP random perturbation and the gradient approximation error of the zeroth-order method, and its effect on fine-tuning trajectory. We provide theoretical analysis for both proposed methods. We conduct extensive empirical analysis on both encoder-only masked language model and decoder-only autoregressive language model, achieving impressive results in terms of scalability and utility regardless of the class of tasks (compared with DPZero, DP-ZOPO improves $4.5\%$ on SST-5, $5.5\%$ on MNLI with RoBERTa-Large and 9.2\% on CB, 3.9\% on BoolQ with OPT-2.7b when $\epsilon=4$, demonstrates more significant enhancement in performance on more complicated tasks).

==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> notations.tex <==
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
% \newtheorem{claim}{Claim}
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{fact}{Fact}[section]
% \theoremstyle{definition}
% \newtheorem{condition}{Condition}[section]
% \newtheorem{definition}{Definition}[section]
% \newtheorem{example}{Example}
% \theoremstyle{remark}
% \newtheorem{remark}{Remark}
% \newtheorem{discussion}{Discussion}[section]
% \newtheorem{fact}{Fact}[section]
\newtheorem{proof}{Proof}[section]
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{fact}{Fact}
% \theoremstyle{definition}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{discussion}{Discussion}

% Jamie bar commend
\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xbar[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother


% \newcommand{\theHalgorithm}{\arabic{algorithm}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\tens}[1]{\boldsymbol{\mathscr{#1}}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
\newcommand{\pgrad}[1]{ \frac{\partial}{\partial{#1} }}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argsup}{\mathop{\rm argsup}}

\newcommand{\fft}{ \mbox{\tt fft} }
\newcommand{\ifft}{ \mbox{\tt ifft} }
\newcommand{\svd}{ \mbox{\tt svd} }

\newcommand{\Unif}{\textrm{Unif}}
% \newcommand{\abs}[1]{\left|{#1}\right|}
% \newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\fnorm}[1]{\|{#1}\|_{\text{F}}}
\newcommand{\infnorm}[1]{\|{#1}\|_\infty}
\newcommand{\spnorm}[2]{\left\| {#1} \right\|_{\text{S}({#2})}}
\newcommand{\sigmin}{\sigma_{\min}}
\newcommand{\tr}{\text{tr}}
\newcommand{\defeq}{\stackrel{\textrm{def}}{=}}
\renewcommand{\det}{\text{det}}
\newcommand{\rank}{\text{rank}}
\newcommand{\logdet}{\text{logdet}}
\newcommand{\trans}{^{\top}}
\newcommand{\poly}{\text{poly}}
\newcommand{\polylog}{\text{polylog}}
\newcommand{\st}{\text{s.t.~}}
\newcommand{\proj}{\mathcal{P}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rdd}{\mathbb{R}^{d\times d}}
\newcommand{\Var}{\text{Var}}

\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}


%%tensors X=L+E A=USV^H
\newcommand{\tA}{\tens{A}}
\newcommand{\tT}{\tens{T}}
\newcommand{\tB}{\tens{B}}
\newcommand{\tC}{\tens{C}}
\newcommand{\tD}{\tens{D}}
\newcommand{\tX}{\tens{X}}
\newcommand{\tL}{\tens{L}}
\newcommand{\tE}{\tens{E}}
\newcommand{\tU}{\tens{U}}
\newcommand{\tV}{\tens{V}}
\newcommand{\tS}{\tens{S}}
\newcommand{\tVH}{\tens{V}^{\mathbf{H}}}
\newcommand{\tM}{\tens{M}}
\newcommand{\tJ}{\tens{J}}
\newcommand{\tG}{\tens{G}}
\newcommand{\tI}{\tens{I}}
\newcommand{\tQ}{\tens{Q}}

\newcommand{\tO}{\tens{O}}

\newcommand{\tY}{\tens{Y}}

\newcommand{\td}{{\tt D}_{\w\w}}
% \newcommand{\htX}{\widehat{\tX}}
% \newcommand{\htY}{\widehat{\tY}}
% \newcommand{\htA}{\widehat{\tA}}
% \newcommand{\htB}{\widehat{\tB}}
% \newcommand{\htT}{\widehat{\tT}}
% \newcommand{\htL}{\widehat{\tL}}
% \newcommand{\htG}{\widehat{\tG}}
% \newcommand{\htU}{\widehat{\tU}}
% \newcommand{\htS}{\widehat{\tS}}
% \newcommand{\htV}{\widehat{\tV}}

% \newcommand{\htX}{\tX_\mathscr{F}}
% \newcommand{\htY}{\tY_\mathscr{F}}
% \newcommand{\htA}{\tA_\mathscr{F}}
% \newcommand{\htB}{\tB_\mathscr{F}}
% \newcommand{\htT}{\tT_\mathscr{F}}
% \newcommand{\htL}{\tL_\mathscr{F}}
% \newcommand{\htG}{\tG_\mathscr{F}}
% \newcommand{\htU}{\tU_\mathscr{F}}
% \newcommand{\htS}{\tS_\mathscr{F}}
% \newcommand{\htV}{\tV_\mathscr{F}}

\newcommand{\fracpar}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

% \newcommand{\A}{\mat{A}}
% \newcommand{\B}{\mat{B}}
% \newcommand{\C}{\mat{C}}
% \renewcommand{\S}{\mat{S}}
% \newcommand{\I}{\mat{I}}
% \newcommand{\M}{\mat{M}}
% \newcommand{\D}{\mat{D}}
% \renewcommand{\P}{\mat{P}}
% \newcommand{\mQ}{\mat{Q}}
% \newcommand{\mR}{\mat{R}}


% \newcommand{\U}{\mat{U}}
% \newcommand{\V}{\mat{V}}
% \newcommand{\W}{\mat{W}}
\newcommand{\X}{\mat{X}}
% \newcommand{\Y}{\mat{Y}}
% \newcommand{\mZ}{\mat{Z}}
% \newcommand{\mSigma}{\mat{\Sigma}}
% \newcommand{\G}{\mat{G}}

% \newcommand{\mU}{\mat{U}}
% \newcommand{\mV}{\mat{V}}
\renewcommand{\S}{\mat{S}}

\renewcommand{\O}{\mat{O}}
\newcommand{\Q}{\mat{Q}}
\newcommand{\E}{\mat{E}}
\renewcommand{\H}{\mat{H}}

%%matrices X=L+E
% \newcommand{\mX}{\mat{X}}
% \newcommand{\mL}{\mat{L}}
% \newcommand{\mE}{\mat{E}}
% \newcommand{\mM}{\mat{M}}
% \newcommand{\mA}{\mat{A}}
% \newcommand{\mB}{\mat{B}}
% \newcommand{\mC}{\mat{C}}
% \newcommand{\mT}{\mat{T}}
% \newcommand{\mY}{\mat{Y}}

% %%matrices bar X=L+E
% \newcommand{\bmX}{\xbar{\mX}}
% \newcommand{\bmL}{\xbar{\mL}}
% \newcommand{\bmE}{\xbar{\mE}}
% \newcommand{\bmM}{\xbar{\mM}}
% \newcommand{\bmA}{\xbar{\mA}}

% \newcommand{\bmY}{\xbar{\mY}}
% \newcommand{\bmU}{\xbar{\U}}
% \newcommand{\bmV}{\xbar{\V}}
% \newcommand{\bmG}{\xbar{\G}}

% \newcommand{\hmM}{\widehat{\mM}}
% \newcommand{\hmY}{\widehat{\mY}}
% \newcommand{\hmA}{\widehat{\mA}}
% \newcommand{\hmU}{\widehat{\U}}
% \newcommand{\hmV}{\widehat{\V}}
% \newcommand{\hmB}{\widehat{\mB}}
% \newcommand{\hmT}{\widehat{\mT}}
% \newcommand{\hmG}{\widehat{\G}}


% \newcommand{\hmM}{\mM_\mathscr{F}}
% \newcommand{\hmY}{\mY_\mathscr{F}}
% \newcommand{\hmA}{\mA_\mathscr{F}}
% \newcommand{\hmU}{\U_\mathscr{F}}
% \newcommand{\hmV}{\V_\mathscr{F}}
% \newcommand{\hmB}{\mB_\mathscr{N}}
% \newcommand{\hmT}{\mT_\mathscr{F}}
% \newcommand{\hmG}{\G_\mathscr{F}}


\newcommand{\vectsigma}{\bm{\sigma}}

\newcommand{\mLambda}{\mat{\Lambda}}
\newcommand{\e}{\vect{e}}
\renewcommand{\u}{\vect{u}}
\renewcommand{\v}{\bm{\nu}}
\newcommand{\vt}{\bm{\nu}_{t}}
\newcommand{\vtpp}{\bm{\nu}_{t+1}}
\newcommand{\p}{\vect{p}}
\newcommand{\g}{\vect{g}}
\renewcommand{\a}{\vect{a}}
\newcommand{\w}{\bm{\omega}}
\newcommand{\wu}{\bm{\omega}^u}
\newcommand{\vdelta}{\bm{\delta}}
\newcommand{\wt}{\bm{\omega}_{t}}
\newcommand{\wtpp}{\bm{\omega}_{t+1}}
\newcommand{\wk}{\bm{\omega}^{k-1}}
\newcommand{\wkpp}{\bm{\omega}^{k}}
\newcommand{\wtk}{\bm{\omega}_t^{k-1}}
\newcommand{\x}{\vect{x}}
\newcommand{\y}{\vect{y}}
\newcommand{\z}{\vect{z}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}

\newcommand{\ur}{\tt{u}}
\newcommand{\UR}{\tt{U}}

\newcommand{\qr}{\tt{q}}
\newcommand{\QR}{\tt{Q}}

\newcommand{\FS}{F_{\tens{S}}}
\newcommand{\FE}{F_{\mathbb{E}}}

% \newcommand{\vw}{\bm{\omega}}
% \newcommand{\vv}{\bm{\nu}}

\newcommand{\RA}{\bm{\mathcal{A}}}


% \newcommand{\tU}{\tilde{\U}_t}
% \newcommand{\tV}{\tilde{\V}_t}
% \newcommand{\tX}{\tilde{\X}}
% \newcommand{\tY}{\tilde{\Y}}
% \newcommand{\tx}{\tilde{\x}}
% \newcommand{\ty}{\tilde{\y}}

% \renewcommand{\L}{\mathcal{L}}

\newcommand{\cn}{\kappa}
\newcommand{\nn}{\nonumber}
\newcommand{\order}[1]{O(#1)}
% \newcommand{\M}{\mat{M}}
% \newcommand\Mmh{\mat{M}^{-1/2}}
% \newcommand{\A}{\mat{A}}
% \newcommand{\B}{\mat{B}}
% \newcommand{\C}{\mat{C}}
% \newcommand{\Et}[1][t]{\mat{E_{#1}}}
% \newcommand{\Etp}{\Et[t+1]}
% \newcommand{\Errt}[1][t]{\mat{\bigtriangleup_{#1}}}
% \newcommand\cnM{\kappa}
% \newcommand{\cn}[1]{\kappa\left(#1\right)}
% \newcommand\X{\mat{X}}
% \newcommand\fstar{f_*}
% \newcommand\Xt[1][t]{\mat{X_{#1}}}
% \newcommand\ut[1][t]{{u_{#1}}}
% \newcommand\Xtinv{\inv{\Xt}}
% \newcommand\Xtp{\mat{X_{t+1}}}
% \newcommand\Xtpinv{\inv{\left(\mat{X_{t+1}}\right)}}
% \newcommand\U{\mat{U}}
% \newcommand\UTr{\trans{\mat{U}}}
% \newcommand{\Ut}[1][t]{\mat{U_{#1}}}
% \newcommand{\Utinv}{\inv{\Ut}}
% \newcommand{\UtTr}[1][t]{\trans{\mat{U_{#1}}}}
% \newcommand\Utp{\mat{U_{t+1}}}
% \newcommand\UtpTr{\trans{\mat{U}_{t+1}}}
% \newcommand\Utptild{\mat{\widetilde{U}_{t+1}}}
% \newcommand\Us{\mat{U^*}}
% \newcommand\UsTr{\trans{\mat{U^*}}}
% \newcommand{\Sigs}{\mat{\Sigma}}
% \newcommand{\Sigsmh}{\Sigs^{-1/2}}
% \newcommand{\eye}{\mat{I}}
% \newcommand{\twonormbound}{\left(4+\DPhi{\M}{\Xt[0]}\right)\twonorm{\M}}
% \newcommand{\lamj}{\lambda_j}

% \renewcommand\u{\vect{u}}
% \newcommand\uTr{\trans{\vect{u}}}
% \renewcommand\v{\vect{v}}
% \newcommand\vTr{\trans{\vect{v}}}
% \newcommand\w{\vect{w}}
% \newcommand\wTr{\trans{\vect{w}}}
% \newcommand\wperp{\vect{w}_{\perp}}
% \newcommand\wperpTr{\trans{\vect{w}_{\perp}}}
% \newcommand\wj{\vect{w_j}}
% \newcommand\vj{\vect{v_j}}
% \newcommand\wjTr{\trans{\vect{w_j}}}
% \newcommand\vjTr{\trans{\vect{v_j}}}

% \newcommand{\DPhi}[2]{\ensuremath{D_{\Phi}\left(#1,#2\right)}}
% \newcommand\matmult{{\omega}}

